Benchmarking Large Language Model Capabilities for Conditional Generation

Pre-trained large language models (PLMs) underlie most new developments in natural language processing. They have shifted the field from application-specific model pipelines to a single model that is adapted to a wide range of tasks. Autoregressive PLMs like GPT-3 or PaLM, alongside techniques like few-shot learning, have additionally shifted the output modality to generation instead of classification or regression. Despite their ubiquitous use, the generation quality of language models is rarely evaluated when these models are introduced. Additionally, it is unclear how existing generation tasks--while they can be used to compare systems at a high level--relate to the real world use cases for which people have been adopting them. In this work, we discuss how to adapt existing application-specific generation benchmarks to PLMs and provide an in-depth, empirical study of the limitations and capabilities of PLMs in natural language generation tasks along dimensions such as scale, architecture, input and output language. Our results show that PLMs differ in their applicability to different data regimes and their generalization to multiple languages and inform which PLMs to use for a given generation task setup. We share best practices to be taken into consideration when benchmarking generation capabilities during the development of upcoming PLMs.

==> notes <==

Todo: 

Show examples/results from Q1 Q2 Q3 ...

Human eval

Question generation 
Surfaces relevant questions that needs to be answered. 
Show examples from Aquamuse? 



Ablations 
Figures 
Examples: Summscreen 4


==

Ayal Klein

I've read through most of your arxiv paper "Conditional Generation with a Question-Answering Blueprint" (very nice work!), and wanted to point your attention to a slight mistake when referencing the QA-SRL paradigm in the related work section. You are referencing two works (QuASE- He et al 2020; Ask it all - Pyatkin et al 2021) that indeed build on to QA-SRL, among other works that extend or utilize the paradigm, some of which you refer later in the section and some you don't (e.g. Large-scale QASRL- FitGeralds et al, 2018; QASRL for nominalizations- Klein et al, 2020; see qasrl.org for more). But the pioneering work first introducing QA-SRL is Question-Answer Driven Semantic Role Labeling: Using Natural Language to Annotate Natural Language. This is the work to cite when referring generally to QA-SRL.  




==

Related work

Generating QA briefs.
https://arxiv.org/pdf/2011.05448.pdf

% T5 (1024x256) 
% LongT5 (4096x256) 
% LongT5 (4096x512)
% E2E (4096x512, sort-rheme-coverage)
% AnswerPlan (Multitasking, 4096x512, sort-rheme-and-lex-cover)
% % AnswerPlan (Multitasking 4096x512 sort-rheme-and-reverse-lex-cover)
% Iterative (4096x512, sort-rheme-coverage, length-constrained)
% Iterative (4096x512 sort-rheme-coverage Q1)
% E2E-filtered (4096x512, sort-rheme-coverage)
% AnswerPlan-filtered (Multitasking, 4096x512, sort-rheme-and-lex-cover)
% Iterative-filtered (4096x512, sort-rheme-coverage, length-constrained)

==

Todo:

Add tags in the table. 


\begin{figure}[t!]
  \footnotesize
  \center{

  }
  \vspace{-0.2cm}
   \caption{Input and target length distributions in different datasets. 
   \label{fig:blueprint-variants}}
  \vspace{-0.5cm}
\end{figure}

